AugGen: Synthetic Augmentation using Diffusion Models Can Improve Recognition

The increasing reliance on large-scale datasets in machine learning poses significant privacy and ethical challenges, particularly in sensitive domains such as face recognition. Synthetic data generation offers a promising alternative; however, most existing methods depend heavily on external datasets or pre-trained models, increasing complexity and resource demands. In this paper, we introduce AugGen, a self-contained synthetic augmentation technique. AugGen strategically samples from a class-conditional generative model trained exclusively on the target FR dataset, eliminating the need for external resources. Evaluated across 8 FR benchmarks, including IJB-C and IJB-B, our method achieves 1-12% performance improvements, outperforming models trained solely on real data and surpassing state-of-the-art synthetic data generation approaches, while using less real data. Notably, these gains often exceed those from architectural enhancements, underscoring the value of synthetic augmentation in data-limited scenarios. Our findings demonstrate that carefully integrated synthetic data can both mitigate privacy constraints and substantially enhance recognition performance. Paper website: https://parsa-ra.github.io/auggen/.

==> sec/method_back2.tex <==

\section{Methodology}\label{sec:method}

\begin{wrapfigure}{r}{0.6\textwidth}  % “r”=right side, width=0.5 of text
    \vspace{-3em}
    \centering
    \includegraphics[width=1.0\linewidth]{sec/imgs/overview_method.drawio.png}
    \caption{
        Overview diagram of AugGen: (a) A labeled dataset, $\mathrm{D}^{\mathrm{orig}}$, is used to train a class-conditional generator, $G(\tZ, \vc)$, and a discriminative model, $\mathrm{M}_{\mathrm{orig}}$. (b,d) Reproduced dataset, $\mathrm{D}^{\mathrm{repro}}$, closely mimics $\mathrm{D}^{\mathrm{orig}}$ under the original conditions. (c) We find new condition vectors, $\mC^{*}$, to generate an augmented dataset, $\mathrm{D}^{\mathrm{aug}}$, using the generator. (f) Augmenting $\mathrm{D}^{\mathrm{orig}}$ with $\mathrm{D}^{\mathrm{aug}}$ boosts $\mathrm{M}{\mathrm{orig}}$ performance without auxiliary datasets or models.
    }
    \label{fig:overview_auggen}
\end{wrapfigure}


% We provide an overview of our proposed methodology in \autoref{fig:overview_auggen}. The core of our approach is to use the features of a discriminator $\mathrm{M}_{\mathrm{orig}}$ and the synthesized images of a generator $G$, to set the conditions of the, $G$ in a way that the resulting images can be used for augmenting the original dataset by treating them as new classes.
% \autoref{fig:overview_auggen} provides an overview of our proposed methodology. Our approach involves using the features from a discriminator $\mathrm{M}_{\mathrm{orig}}$, and the generated images from a generator $G$, both trained on a single dataset. We condition $G$ so that the generated images can be treated as new classes, effectively augmenting the original dataset.
% First, we outline a general problem formulation for both the discriminator (Classifier Training and its output) and the generator (Generator Training block and its output) in \autoref{sec:disc_method} and \autoref{sec:genmodel_method} respectively. We then present our main contribution: generating new classes (Finding Weights in Figure. 3(c)) to augment real datasets with the generated images in the latter. 

\autoref{fig:overview_auggen} illustrates our approach, where a discriminator $\mathrm{M}_{\mathrm{orig}}$ and a generator $G$ are trained on the same dataset. By strategically sampling from $G$, we generate synthetic images forming new classes, augmenting the original dataset. We first define the problem for the discriminator and generator in \autoref{sec:disc_method} and \autoref{sec:genmodel_method}, then introduce our key contribution: generating new classes (Finding Weights, \autoref{fig:overview_auggen}(c)) to complement real datasets with synthetic images.
%Overview diagram of AugGen, (a) we used a single labeled dataset, $\mathrm{D}^{\mathrm{orig}}$, for training a class-conditional generator, $G(\tZ, \vc)$ and also a discriminative model, $\mathrm{M}_{\mathrm{orig}}$. (b,d) If we set the conditions as it was trained in a class-conditional way, we are closely reproducing the original dataset, depicted as $\mathrm{D}^{\mathrm{repro}}$. Later (c) with both of these models, we find new condition vectors, $\mC^{*}$ that will lead to a new dataset, $\mathrm{D}^{\mathrm{aug}}$ (when we are giving the new condition to the generator and sampling from it). The conditions are set in a way that the newly generated dataset would be beneficiary for boosting the performance of the $\mathrm{M}_{\mathrm{orig}}$ when we augment it with the original dataset (f). This is done without relying on any auxiliary dataset/model.


\subsection{Discriminative Model}\label{sec:disc_method}
% Assume that we have a dataset, $\mathbf{D}_{\mathrm{orig}}$, consist of $\mathrm{k}$ pairs of image and labels, $\{(\tX_0, y_0), (\tX_1, y_1), \dots, (\tX_\mathrm{k-1}, y_\mathrm{k-1}) \}$. $\tX_\mathrm{i}$ is an image of the form $\R^{\mathrm{H}\times\mathrm{W}\times3}$, for simplicity here we assume that the $\mathrm{H}$ and $\mathrm{W}$ are fixed for all of the $k$ sample pairs in our dataset. $y_i$ is a scalar that depicts the label of images from a fixed set of $l$ possible values (\emph{e.g.,} $\{0, 1, ..., l-1\}$), $\sL$, which $l < \mathrm{k}$. Here the goal of a discriminative model is to learn the conditional probability $p( \vy | \tX )$ using the samples in $\mathbf{D}^{\mathrm{orig}}$. For example here the $\mathbf{D}^\mathrm{orig}$ can be the ImageNet~\cite{imagenet15russakovsky} or CASIA-WebFace~\cite{casiawebface} dataset. The discriminative model's task is to identify the most likely class of the image. In most cases this enforces the features (\emph{i.e.}, usually the output of penultimate layer, $\ve$)  for the similar images to be closer together according to a measure, $m$ (\emph{e.g.}, Cosine Distance, the lower the output of $m(\ve_1, \ve_2)$ the more similar the features $\ve_1$ and $\ve_2$ are). This is usually learned by a mapping function $f_{\theta_{\mathrm{dis}}}: \tX \rightarrow \vy $ parameterized by $\theta_{\mathrm{dis}}$ which uniquely describes the architecture and the parameters of the $f$. The $\theta_{\mathrm{dis}}$ is learned through empirical risk minimization as follows: 

% \begin{equation}
%     \theta_{\mathrm{dis}}^* = \underset{\theta_\mathrm{dis} \in \Theta_{\mathrm{dis}}}{argmin} \hspace{5pt} \E_{(\tX, y) \sim \mathrm{D}^{\mathrm{orig}}}[\mathcal{L}_{\mathrm{dis}}(f_{\theta_\mathrm{dis}}(\tX), \vy)] 
% \end{equation}

% Where for a classification problem the, $\mathcal{L}_{\mathrm{dis}}$, is usually in the form of Cross-Entropy and the Expectation here is being calculated by drawing sample pairs from, $\mathbf{D}^{\mathrm{orig}}$. Here we refer to possible hyperparameters for calculating the $\theta_{\mathrm{dis}}^{*}$ as $\mathrm{h}_{\mathrm{dis}}$, which tries to abstract out the processes such as learning rates and its schedules, the number of training epochs and other details involved in training a neural network for real-world applications. As depicted in \autoref{fig:overview_auggen}(a), The outcome of this process is a model, $\mathrm{M}_{\mathrm{orig}}$, (\emph{i.e.}, $f_{\theta_\mathrm{{dis}^{*}}}$), which tries to reflect that the model is trained on the $\mathbf{D}_\mathrm{orig}$.

Assume a dataset $\mathbf{D}_{\mathrm{orig}} = \{(\tX_i, y_i)\}_{i=0}^{k-1}$, where each $\tX_i \in \R^{H\times W\times 3}$ and $y_i \in \{0,\dots,l-1\}$ ($l < k$). The goal is to learn a discriminative model $f_{\theta_{\mathrm{dis}}}: \tX \rightarrow \vy$ that estimates $p(\vy|\tX)$ (e.g., on ImageNet~\cite{imagenet15russakovsky} or CASIA-WebFace~\cite{casiawebface}). Typically, similar images have closer features under a measure $m$ (e.g., cosine distance). We train $f_{\theta_{\mathrm{dis}}}$ via empirical risk minimization:
\vspace{-0.5em}
\begin{equation}
    \theta_{\mathrm{dis}}^* 
    = \underset{\theta_\mathrm{dis} \in \Theta_{\mathrm{dis}}}{\arg\min}
    \, \E_{(\tX, y) \sim \mathbf{D}_{\mathrm{orig}}}
    \bigl[\mathcal{L}_{\mathrm{dis}}(f_{\theta_{\mathrm{dis}}}(\tX), \vy)\bigr],
\end{equation}

where $\mathcal{L}_{\mathrm{dis}}$ is typically cross-entropy, and $\mathrm{h}_{\mathrm{dis}}$ denotes hyperparameters (e.g., learning rates). The resulting model $\mathrm{M}_{\mathrm{orig}} = f_{\theta_{\mathrm{dis}}^*}$ is shown in \autoref{fig:overview_auggen}(a).


\subsection{Generative Model}\label{sec:genmodel_method}

% Generative models aim to capture the underlying distribution of the dataset given some samples, such that new samples can be drawn from it. Here we present general problem formulation in the context of the diffusion models, in which we also demonstrate the experiments using these types of models in \autoref{sec:exps}. Diffusion models \cite{song2020denoising, anderson1982reverse_diff} operate by incrementally adding noise to data (\emph{i.e.}, $\tX_i$s) and training a denoiser or score function, $\mathrm{S}$.  This is done to gradually learn to go from a complete white Gaussian noise (\emph{i.e.}, in the sampling process) to the data distribution, by adding noise to the data in different scales and learning the noise that was added to the data during the training process (\emph{i.e.}, supervision). Following~\cite{Karras2024edm2, karras2022elucidating} formulation, $\mathrm{S}$, the denoiser function can be learned in two stages. The first stage is that given a noise level, $\sigma$, we optimize the parameters of the denoiser (\emph{i.e.}, $\theta_{\mathrm{den}}$) by adding a noise $\tN^{h \times w \times c}$ which is dependent on $\sigma$ and removing it by the denoiser function as follows:

% \begin{equation}
% \begin{aligned}
%      \mathcal{L}(S_{\theta_{den}};\sigma) &= \E_{(\tX,y) \sim \mathrm{D}^{\mathrm{orig}}, \tN \sim \mathcal{N}(\mathbf{0}, \sigma\tI)}\\&[|| \mathrm{S}_{\theta_{den}}(E_{\mathrm{VAE}}(\tX) + \tN; \mathrm{c}(y), \sigma ) - \tX ||^{2}_{2} ]
%      \label{eq:den_stage_1}
% \end{aligned}
% \end{equation}

% Here the image and its corresponding label, $(\tX,y)$ are sampled from, $\mathrm{D}^{\mathrm{orig}}$. Then the $\tX$ is \emph{optionally} passed to a VAE encoder, $\tZ^{h \times w \times c} = E_{\mathrm{VAE}}(\tX)$ in case we are working on the latent diffusion paradigm \cite{rombach2022high_ldm} (\emph{i.e.,} we will show experiments for both pixel and latent based diffusion). Later this $\tZ$ can be transformed back to image space using the VAE's decoder, $\tX \simeq D_{\mathrm{VAE}}(E_{\mathrm{VAE}}(\tX))$.
%  Latent diffusion models are mostly popular because of lower computational cost with respect to pixel-level diffusion models, especially in higher resolution. The denoising is done in the latent space of the VAE and later decoded to the pixel space.  
% The denoiser function takes the noisy input, noise scale, and the class condition, $c(y)$ as input and tries to estimate the original latent, $E_{\mathrm{VAE}}(\tX)$, or image, $\tX$. The second stage is to iterate over different data-dependent noise scales which reduces the final optimization target to: 

% \begin{equation}
%     \theta_{den}^{*} = \underset{\theta_{den} \in \Theta_{den}}{argmin} \E_{\sigma \sim \mathcal{N}(\mu,\sigma^2)}  [\lambda_{\sigma} \mathcal{L}(\mathrm{S}_{\theta_{den}};\sigma) ]
%     \label{eq:den_stage_2}
% \end{equation}

% Where $\lambda_{\sigma}$ is noise scale dependent weight, and $\mu$ and $\sigma$ in $\mathcal{N}(\mu, \sigma^2)$ are empirically set to focus the training on more important noise levels beneficiary for denoiser \cite{Karras2024edm2,karras2022elucidating}.

Generative models seek to learn the data distribution, enabling the generation of new samples. We use diffusion models~\cite{song2020denoising,anderson1982reverse_diff}, which progressively add noise to data and train a denoiser $\mathrm{S}$. Following \cite{karras2022elucidating,Karras2024edm2}, $\mathrm{S}$ is learned in two stages. First, for a given noise level $\sigma$, we add noise $\tN$ to $E_{\mathrm{VAE}}(\tX)$ (or $\tX$ directly in pixel-based diffusion) and remove it via:
\begin{equation}
\begin{aligned}
    \mathcal{L}(S_{\theta_{den}};\sigma) &= \E_{(\tX,y)\sim \mathrm{D}^{\mathrm{orig}}, \tN \sim \mathcal{N}(\mathbf{0}, \sigma\tI)}\\
    &\left[\| \mathrm{S}_{\theta_{den}}(E_{\mathrm{VAE}}(\tX) + \tN; \mathrm{c}(y), \sigma ) - \tX \|^{2}_{2}\right],
\end{aligned}
\label{eq:den_stage_1}
\end{equation}
where $\mathrm{c}(y)$ denotes the class condition, and $E_{\mathrm{VAE}}(\cdot)$ and $D_{\mathrm{VAE}}(\cdot)$ are optional VAE encoder and decoder. In the second stage, we sample different noise levels and minimize:
\begin{equation}
    \theta_{den}^{*} = \underset{\theta_{den} \in \Theta_{den}}{\arg\min} \,
    \E_{\sigma \sim \mathcal{N}(\mu,\sigma^2)} 
    \bigl[\lambda_{\sigma} \,\mathcal{L}(\mathrm{S}_{\theta_{den}};\sigma)\bigr],
\label{eq:den_stage_2}
\end{equation}

where $\lambda_{\sigma}$ weights each noise scale. Latent diffusion~\cite{rombach2022high_ldm} conducts denoising in a compressed latent space, reducing computational cost for high-resolution data.


\subsection{Class Mixing}\label{sec:class_mixing}

% In our formulation, we used one-hot encoding for the $c$ function, meaning that, if the dataset $\mathrm{D}^{\mathrm{orig}}$ contains $l$ unique labels, $c$ maps each $i \in \{0,1,\dots, l\}$ to a unique vector of size $l$ that the value corresponding to the label is 1, while the rest are set to 0, later this vector will be mapped to lower dimensions of the condition space of the denoiser. After training the conditional denoiser (\emph{i.e.}, $\mathrm{S}_{\theta_{\mathrm{den}}}$), using \autoref{eq:den_stage_2}, as depicted in \autoref{fig:overview_auggen}(c), we can sample from the generator in two ways. 
% \begin{enumerate}
%     %\item During sampling, we pass the condition vector, $\vc$, as it was passed to it during the training of, S, (\emph{i.e.}, one-hots corresponding to the classes).
%     \item During sampling, we set the condition vector $\vc$ as it was during the training of $\mathrm{S}$, i.e., one-hot vectors representing the classes.
%     \item The condition $\vc^{*}$ is different from the values that were used during the training of the generator.
%     %The condition $\vc^{*}$, is not like the type that we trained our model with.
% \end{enumerate}

% As an example, depicted in \autoref{fig:overview_auggen}(d), when we pass $\vc$, one-hot condition vector corresponding to the first class, we expect the generator to synthesize samples that are highly similar to the first class in the, $\mathrm{D}^{\mathrm{orig}}$. We refer to this dataset that tries to reproduce the, $\mathrm{D}^{\mathrm{orig}}$, the $\mathrm{D}^{\mathrm{repro}}$. In this work, we explored 
% %the second way 
% the ways of conditioning a generator with the values that it has not seen before, and how we can use the model  $\mathrm{M}_{\mathrm{orig}}$ that was trained using the dataset $\mathrm{D}^{\mathrm{orig}}$ to generate samples that can be used to make $\mathrm{M}_{\mathrm{mix}}$ more robust (\emph{i.e.}, consistently more performing in various benchmarks). As mentioned previously, 
% our goal is to synthesize a new class by combining two conditions that the generator has seen before (\emph{i.e.}, the one-hot condition during training). As depicted in \autoref{fig:explain_dynamics_intro}, we want the new class to be between two or more source classes so that we can enhance the inter-class separation and increase the compactness even further. 


In our formulation, $c$ is one-hot encoded for each label in $\mathrm{D}^{\mathrm{orig}}$, then mapped to the denoiser's condition space. After training the conditional denoiser $\mathrm{S}_{\theta_{\mathrm{den}}}$ (\autoref{fig:overview_auggen}, (c)) via \autoref{eq:den_stage_2}, we can sample from the generator in two ways:
\begin{enumerate}
    \item Use the same one-hot vectors as in training, producing samples similar to $\mathrm{D}^{\mathrm{orig}}$. As an example, when passing the one-hot vector for the first class, the generator synthesizes samples that resemble this class (\autoref{fig:overview_auggen}, (d)), collectively forming $\mathrm{D}^{\mathrm{repro}}$.
    \item Apply novel condition vectors $\vc^{*}$ different from those used during training.
\end{enumerate}
We explore combining known conditions to synthesize entirely new classes, aiming to increase inter-class separation and feature compactness as presented in \autoref{fig:explain_dynamics_intro}. By leveraging the previously trained $\mathrm{M}_{\mathrm{orig}}$, these additional samples can make $\mathrm{M}_{\mathrm{mix}}$ (\emph{i.e.}, discriminator trained on the mix of real and generated data) better across diverse benchmarks.

% Our target is by using some combination of two conditions that the generator has seen before (\emph{i.e.}, the one-hot condition during training) we could synthesize a hypothetically new class that will benefit the training of, $\mathrm{M}$. 

% To this end, given the one-hot condition of two classes, $i$ and $j$, namely, $\vc^{\mathrm{i}}$ and $\vc^{\mathrm{j}}$, we seek to find $\alpha$ and $\beta$ such that the condition vector of a  hypothetically new class would be: 

% \begin{equation}
%     \vc^{*} = \alpha \vc^{\mathrm{i}} + \beta \vc^{\mathrm{j}}
%     \label{eq:opt_weight_construction}
% \end{equation}

% For ease of notation here we denote the generation process of the trained denoiser by a function $G$, $ \tX^{i} = G(\tZ, \vc^{i})$, which involves giving as input the $\tZ \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ and condition vector $\vc$ to the generator to denoise the noisy input. Later optionally, we decode the result using $D_{\mathrm{VAE}}$ back to the image space (\emph{i.e.}, in case we are working with latent diffusion models). For finding the $\alpha$ and $\beta$ that produces a class that is dissimilar to the source classes that we are mixing (\emph{i.e.}, $i$ and $j$ in \autoref{eq:opt_weight_construction}) and also similar within each other (\emph{i.e.}, when we give the same condition to $G$ we expect the model to generate images of the same class) we formulate the problem as a search grid. 
\vspace{-0.5em}
Given two classes $i$ and $j$ with one-hot vectors $\vc^{\mathrm{i}}$ and $\vc^{\mathrm{j}}$, we construct a new class condition via
\begin{equation}
    \vc^{*} = \alpha \vc^{\mathrm{i}} + \beta \vc^{\mathrm{j}},
    \label{eq:opt_weight_construction}
\end{equation}
We denote the trained denoiser's generation process by $G$, so $\tX^i = G(\tZ, \vc^i)$ uses noise $\tZ \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ and condition $\vc$ to iteratively denoise the input.
%We denote the generator (denoiser) by $G$, such that $\tX = G(\tZ, \vc)$ for $\tZ \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$, optionally decoding $\tX$ via $D_{\mathrm{VAE}}$ in latent diffusion. 
To find suitable $\alpha$ and $\beta$, we formulate the problem as a grid search, aiming for dissimilarity to classes $i$ and $j$ while preserving class coherence for repeated samples from $G(\tZ, \vc^{*})$. We set the $\alpha$ and $\beta$ to some possible combinations in a linear space of the values between $0.1$ to $1.1$. For example, possible combinations would be $\alpha = 0.3 , \beta = 0.5$ or $\alpha = 1.1, \beta = 0.4$. We denote $\sW$, the set which contains possible values of $\alpha$ and $\beta$. We also select some subset of $\sL$ and call it $\sL_{s}$, for the set to contain some specific classes. Then we randomly select two values from the $\sL_{s}$ namely $i$ and $j$. Later for each  $(\alpha, \beta) \in \sW $ we apply the \autoref{eq:opt_weight_construction}, to get the $\vc^{*}$. We generate three types of images. The first two is the reproduction dataset, $\mathrm{D}^{\mathrm{repro}}$ as before by setting the conditions to $\vc^{i}$ and $\vc^{j}$, to get $\tX^{i} = G(\tZ, \vc^{i})$ and $\tX^{j} = G(\tZ, \vc^{j})$.
Finally the third one is $\tX^{*} = G(\tZ, \vc^{*})$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Wrapped version of the plots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\begin{wrapfigure}{r}{0.60\textwidth}
  \vspace{-1.5ex}  
  \captionsetup{type=algorithm}
  \captionof{algorithm}{Grid search for $\alpha$ and $\beta$}
  \label{alg:grid_search}
  \begin{algorithmic}[1]
    \Require Search range for $\alpha, \beta \in [0.1, 1.1]$,$\sL_{s} \subseteq \sL$, $K$: Number of iterations.
    \Require $G(.,.)$: Class-conditional Generator trained on $\mathrm{D}^{\mathrm{orig}}$
    \Require $f_{\theta_{\mathrm{dis}}^{*}}$: Discriminator trained on $\mathrm{D}^{\mathrm{orig}}$
    
    \textbf{Output:}  $\alpha^*$ and $\beta^*$
    \
    \State Create set $\sW = \{ (\alpha, \beta) \mid \alpha, \beta \in [0.1, 1.1] \}$
    \State Randomly select two values $i$ and $j$ from $\sL_{s}$

    \State Create empty set $\sM$.
    \For{each $(\alpha, \beta) \in \sW$}
        \State $\vc^{*} = \alpha \vc^{\mathrm{i}} + \beta \vc^{\mathrm{j}}$
        
        \State Create empty set $\sF$.
        
        \For{k = $1, \dots, K$ }
            \State Get Repro Images   : $\tX^{i} = G(\tZ, \vc^{i}), \tX^{j} = G(\tZ, \vc^{j})$
            \State Get Interpolated Images : $\tX^{*} = G(\tZ, \vc^{*})$    
            \State Get Repro Features: 
            $\ve^{i}, \ve^{j} = f_{\theta_{\mathrm{dis}}^{*}}(\tX^{i}), f_{\theta_{\mathrm{dis}}^{*}}(\tX^{j})$
            \State Get Interpolated Feature: $  \ve^{*} = f_{\theta_{\mathrm{dis}}^{*}}(\tX^{*}) $
            
            \State Add $\ve^{*}$ to $\sF$
            
            \State Dissimilarity measures: $d_{i} = m_{\mathrm{d}}(\ve^{i}, \ve^{*})$
            \Statex \hspace{125pt} $d_{j} = m_{\mathrm{d}}(\ve^{j}, \ve^{*})$
            \State Total dissimilarity: $m_{\mathrm{d}}^{\mathrm{total}} = |d_{i}| + |d_{j}|$
        \EndFor

        \State $m_{\mathrm{s}}^{\mathrm{total}} = 0 $

        \State $ \forall p,q \in \sF | p \neq q $ Calculate $m_{\mathrm{s}}( \ve^{p}, \ve^{q})$ and add it to $m_{\mathrm{s}}^{\mathrm{total}}$

        \State Final measure: $m^{\mathrm{total}} = m_{\mathrm{s}}^{\mathrm{total}} + m_{\mathrm{d}}^{\mathrm{total}}$ and add it to $\sM$.
    \EndFor
    
    \State Return $\alpha^*$ and $\beta^*$ that the $m^{\mathrm{total}}$, in $\sM$ is high. 
  \end{algorithmic}
  \vspace{-1ex}
\end{wrapfigure}


By passing the generated images to the $f_{\theta_\mathrm{{dis}^{*}}}$ (\emph{i.e.}, our discriminator which was trained on the $\mathrm{D}^{\mathrm{orig}}$) we get the features, $\ve^{i}$, $\ve^{j}$ and $\ve^{*}$ respectively. We seek to maximize the dissimilarity between generated images so that we can treat the new sample $\tX^{*}$ as a new class. For this, we use a dissimilarity measure, $m_{d}$ which the \emph{higher} the absolute value it produces the more dissimilar the inputs are. We calculate this measure for each of the reproduced images of the existing classes with respect to the new class, $d_{i} = m_{\mathrm{d}}(\ve^{i}, \ve^{*})$ and $d_{j} = m_{\mathrm{d}}(\ve^{j}, \ve^{*})$, and we define the total dissimilarity between the reproduced classes and the newly generated class as $m_{\mathrm{d}}^{\mathrm{total}} = |d_{i}| + |d_{j}|$. We repeat this process $K$ times, this means that we get $K$ different $\tX^{*}$ for the same $\vc^{i})$ and $\vc^{j})$. We also want each $K$ $\tX^{*}$ to be as similar as possible to each other so we can assign the same label/class to them for a fixed $\alpha$ and $\beta$. To this end, we also calculate a similarity measure, $m_{s}$, in which the higher the absolute output of this measure is the the more similar their input is. We define the total similarity between the $K$ generated $\tX^{*}$ as $m_{\mathrm{s}}^{\mathrm{total}}$. 
We hypothesize and verify later with our experiments that the good candidates for $\alpha$ and $\beta$ are the ones that have a high value of the $m^{\mathrm{total}} = m_{\mathrm{s}}^{\mathrm{total}} + m_{\mathrm{d}}^{\mathrm{total}} $. This search for $\alpha$ and $\beta$ is outlined in the \autoref{alg:grid_search}.
%This search for $\alpha$ and $\beta$ is presented in the \autoref{alg:grid_search}.
Finally the third one is $\tX^{*} = G(\tZ, \vc^{*})$. By passing the generated images to the $f_{\theta_\mathrm{{dis}^{*}}}$ (\emph{i.e.}, our discriminator which was trained on the $\mathrm{D}^{\mathrm{orig}}$) we get the features, $\ve^{i}$, $\ve^{j}$ and $\ve^{*}$ respectively. We seek to maximize the dissimilarity between generated images so that we can treat the new sample $\tX^{*}$ as a new class. For this, we use a dissimilarity measure, $m_{d}$ which the \emph{higher} the absolute value it produces the more dissimilar the inputs are. We calculate this measure for each of the reproduced images of the existing classes with respect to the new class, $d_{i} = m_{\mathrm{d}}(\ve^{i}, \ve^{*})$ and $d_{j} = m_{\mathrm{d}}(\ve^{j}, \ve^{*})$, and we define the total dissimilarity between the reproduced classes and the newly generated class as $m_{\mathrm{d}}^{\mathrm{total}} = |d_{i}| + |d_{j}|$. We repeat this process $K$ times, this means that we get $K$ different $\tX^{*}$ for the same $\vc^{i})$ and $\vc^{j})$. We also want each $K$ $\tX^{*}$ to be as similar as possible to each other so we can assign the same label/class to them for a fixed $\alpha$ and $\beta$. To this end, we also calculate a similarity measure, $m_{s}$, in which the higher the absolute output of this measure is the the more similar their input is. We define the total similarity between the $K$ generated $\tX^{*}$ as $m_{\mathrm{s}}^{\mathrm{total}}$. 
We hypothesize and verify later with our experiments that the good candidates for $\alpha$ and $\beta$ are the ones that have a high value of the $m^{\mathrm{total}} = m_{\mathrm{s}}^{\mathrm{total}} + m_{\mathrm{d}}^{\mathrm{total}} $. This search for $\alpha$ and $\beta$ is outlined in the \autoref{alg:grid_search}.





%––– Algorithm 2 on its own top–of–page wrap
\clearpage
\noindent
\begin{wrapfigure}{r}{0.48\textwidth}
  \vspace{-1.5ex}  
  \captionsetup{type=algorithm}
  \captionof{algorithm}{Generating $\mathrm{D}^{\mathrm{aug}}$}
  \label{alg:auggen}
  \begin{algorithmic}[1]
    \Require  $\alpha^*$ and $\beta^*$ from \autoref{alg:grid_search}, $\sL_{s} \subseteq \sL$, $C$: Number of mixed classes, $N$: Number of samples per class. 
    \Require $G(.,.)$: Class-conditional Generator trained on $\mathrm{D}^{\mathrm{orig}}$
    
    \textbf{Output:}  $\mathrm{D}^{\mathrm{aug}}$
    \
    \State Create empty set $\mathrm{D}^{\mathrm{aug}}$.
    \For{n = $1, \dots, C$ }
        \State Randomly select two values $i$ and $j$ from $\sL_{s}$
        \State $\vc^{*} = \alpha^{*} \vc^{\mathrm{i}} + \beta^{*} \vc^{\mathrm{j}}$
        \State Create empty set $T$
        \For{n = $1, \dots, N$ }
            \State $\tX^{*} = G(\tZ, \vc^{*})$
            \State Add $\tX^{*}$ to $T$. 
        \EndFor
        \State Add $T$ to $\mathrm{D}^{\mathrm{aug}}$. 
    \EndFor
    
    \State Return $\mathrm{D}^{\mathrm{aug}}$ 
  \end{algorithmic}
  \vspace{-1ex}
\end{wrapfigure}




After finding candidate values for $\alpha$ and $\beta$, by randomly selecting classes from $\sL$, and calculating $\vc^{*}$, we can generate images that represent a hypothetically new class. The output of this process is what we call generated augmentations of the $\mathrm{D}^{\mathrm{orig}}$, or $\mathrm{D}^\mathrm{aug}$ as depicted in the \autoref{fig:overview_auggen} (e) and presented in \autoref{alg:auggen}. 
% As depicted in \autoref{fig:explain_dynamics_intro} since the newly generated classes are similar within each other and yet dissimilar from their mixed classes although they inherently have some ques of their source classes, we expect training with the mix \orig and \aug  (\autoref{fig:overview_auggen} (f)), would be beneficiary for the discriminator. We demonstrated this improvement in the \autoref{sec:exps} by extensive experiments.
As shown in \autoref{fig:explain_dynamics_intro}, the newly generated classes are similar within themselves but distinct from their mixed classes, retaining source-class cues to aid discrimination by design. Training with the mix of \orig and \aug (\autoref{fig:overview_auggen}(f)) benefits the discriminator, as demonstrated in \autoref{sec:exps}.
%(\emph{i.e.}, consistently outperforming discriminative model trained on the)$\mathrm{D}^{\mathrm{orig}}$ in various benchmarks. 
%In the \autoref{app:downstream_performance_vs_gen_metrics} we experimentally show that the usual metrics that are used for quantifying the performance of the generators do not correlate to the final performance of a downstream task.




% \section{Why it works?}\label{sec:intuition}
% An overview of the dynamics of our work is presented in \autoref{fig:explain}. For the baseline, we train a discriminator on the original classes using a margin-based loss, enabling it to distinguish different classes, like M and N using the margin losses reflected in, $\theta_{\mathrm{baseline}}$, and at the same time make the samples of each class as compact as possible. 

% After mixing the conditions of M and N as per \autoref{alg:auggen}, as appeared on the right side of the \autoref{fig:explain}, and treating the mixed identity as a new class while training on top of the $\mathrm{D}^{\mathrm{orig}}$, the network is forced to discriminate between this new mixed class (between M and N), and also the original M and N, leading to a larger cosine distance $\theta_{\mathrm{ours}}$ between M and N. This enhances the discriminative power. This also results in the more compactness of the samples within each class as we are trying to increase the $\theta_{\mathrm{ours}}$. This hypothesis will be verified experimentally in \autoref{sec:exps}. 



